Never Use Labels: Signal Strength-Based Bayesian Device-Free Localization in Changing Environments

Device-free localization (DFL) methods use measured changes in the received signal strength (RSS) between many pairs of RF nodes to provide location estimates of a person inside the wireless network. Fundamental challenges for RSS DFL methods include having a model of RSS measurements as a function of a person's location, and maintaining an accurate model as the environment changes over time. Current methods rely on either labeled empty-area calibration or labeled fingerprints with a person at each location. Both need to be frequently recalibrated or retrained to stay current with changing environments. Other DFL methods only localize people in motion. In this paper, we address these challenges by, first, introducing a new mixture model for link RSS as a function of a person's location, and second, providing the framework to update model parameters without ever being provided labeled data from either empty-area or known-location classes. We develop two new Bayesian localization methods based on our mixture model and experimentally validate our system at three test sites with seven days of measurements. We demonstrate that our methods localize a person with non-degrading performance in changing environments, and, in addition, reduce localization error by 11-51% compared to other DFL methods.

==> Future_Work.tex <==
\section{Future Work}

For parameter estimation:
Why do you run KRTI?
Why do you use euclidean norm instead of KL divergence or Gaussian kernel?
There are fewer RSS measurements the greater the excess path length is. This means the histograms may not represent the true distribution of RSS for the given excess path length. The problem is compounded if shorter training periods or larger areas to walk are used. These issues could result in too few measurements to reliably estimate beta and lambda. An alternative would be to create bins with unequal widths to more even distribute the RSS into the bins.

Use something other than normal distribution. rician or rayleigh

We recognize that we're making the assumption that the affected mean is always less than the unaffected mean and that the affected variance is a scalar multiple of the unaffected variance. This is certainly not always the case for all links. But it is for many links. An alternative way to estimate the affected mean and variance could be to implement a secondary buffer for RSS measured when the link is affected. This way, both the unaffected and affected distribution parameters are estimated independently. However, we leave this to future work. We also note that, although our model is very simplified and may not capture all of the differences in the RSS distribtuions as a function of location, we keep complexity low by only having to estimate two parameters $\hat{\mu}_{l,u}$ and $\hat{\sigma}^2_{l,u}$ for each link. By doing so, we ensure that our system can operate in real-time.

==> paper_header.tex <==
\markboth{IEEE Transactions on Mobile Computing}{}
